Algorithms for group isomorphism via group extensions and cohomology

The isomorphism problem for finite groups of order n (GpI) has long been known to be solvable in $n^{\log n+O(1)}$ time, but only recently were polynomial-time algorithms designed for several interesting group classes. Inspired by recent progress, we revisit the strategy for GpI via the extension theory of groups. The extension theory describes how a normal subgroup N is related to G/N via G, and this naturally leads to a divide-and-conquer strategy that splits GpI into two subproblems: one regarding group actions on other groups, and one regarding group cohomology. When the normal subgroup N is abelian, this strategy is well-known. Our first contribution is to extend this strategy to handle the case when N is not necessarily abelian. This allows us to provide a unified explanation of all recent polynomial-time algorithms for special group classes. Guided by this strategy, to make further progress on GpI, we consider central-radical groups, proposed in Babai et al. (SODA 2011): the class of groups such that G mod its center has no abelian normal subgroups. This class is a natural extension of the group class considered by Babai et al. (ICALP 2012), namely those groups with no abelian normal subgroups. Following the above strategy, we solve GpI in $n^{O(\log \log n)}$ time for central-radical groups, and in polynomial time for several prominent subclasses of central-radical groups. We also solve GpI in $n^{O(\log\log n)}$ time for groups whose solvable normal subgroups are elementary abelian but not necessarily central. As far as we are aware, this is the first time there have been worst-case guarantees on a $n^{o(\log n)}$-time algorithm that tackles both aspects of GpI---actions and cohomology---simultaneously.

==> groupcode.tex <==
\subsection{Group code equivalence over cyclic groups}
For a group $\Gamma$, a \emph{group code of length $n$ over $\Gamma$} or a \emph{$\Gamma$-code of length $n$} is a subgroup of $\Gamma^{n}$. Two $\Gamma$-codes of length $n$ are \emph{equivalent} if there is a permutation of $[n]$ which makes them equal by permuting the $n$ coordinates. As usual for isomorphism-type problems, the set of equivalences between two group codes is either empty or a coset of the automorphism group (=self-equivalences) of one of them. Note that $\F_p$-linear codes---for which a singly exponential-time algorithm was given by Babai (reproduced as Theorem~\ref{thm:code_eq} above)---are the same as group codes over the prime cyclic group over $\Z_p$. The following theorem makes progress on an open question from \cite{BCGQ}:

\begin{theorem} \label{thm:groupcode}
The coset of equivalences of two group codes of length $n$ over the cyclic group $\Z_{m}$, given by generating sets, can be found in $(2 + o(1))^{n}\log^2(m)$ time.

More specifically, equivalence of such codes that are generated by $d$ elements reduces to $\binom{n}{d}$ instances of $d \times (n - d)$ \algprob{Edge-and-Vertex-Colored Bipartite Graph Isomorphism} in time $n^{O(1)}\log^2(m)$ per instance.
\end{theorem}

For Theorem~\ref{thm:groupcode} we replace the use of row echelon form in Babai's algorithm (as explained in \cite[paragraph before Cor.~4.5.2]{grochowPhD}) with a variant of Hermite (row-)normal form that works over principal ideal rings such as $\Z_{m}$ \cite{buchmannNeis}.\footnote{The standard Hermite normal form---as presented, for example, in Cohen's book \cite[Section~2.5]{cohenBook}---is for subgroups of $\Z^{m}$, or more generally modules of principal ideal \emph{domains}---rings without zero-divisors in which every ideal is generated by a single element. Although $\Z_{m}$ has zero-divisors, it is still a principal ideal ring, and furthermore we can choose canonical generators for each ideal---two key properties that allow for the existence, uniqueness, and computation of Hermite normal form. In particular, if we think of the elements of $\Z_{m}$ as represented by integers between $0$ and $m-1$, then we choose as the canonical generator of an ideal the least element in the ideal, under the usual ordering on the integers between $0$ and $m-1$.}

For completeness, we first recall the variant of Hermite normal form that we use, which is a special case of the Hermite normal form for principal ideal rings \cite{buchmannNeis}. Every subgroup of $\Z_{m}$ is cyclic. Given a set of elements $a_1, \dotsc, a_k \in \Z_{m}$, a ``GCD'' of $a_1, \dotsc, a_k$ is any element $g \in \Z_{m}$ such that $\langle g \rangle = \langle a_1, \dotsc, a_m \rangle$, where $\langle \bullet \rangle$ denotes the subgroup generated by $\bullet$. If we think of the elements of $\Z_{m}$ as (represented by) the integers $0, 1, \dotsc, m-1$, then we define the normalized GCD of $a_1, \dotsc, a_k$ to be their smallest GCD under the usual ordering on the integers $0, \dotsc, m-1$. Now, let $M$ be a $d \times n$ matrix over $\Z_{m}$, and suppose that $d'$ is the smallest number of generators of the subgroup of $\Z_{m}^{n}$ generated by the rows of $M$. Then the Hermite normal form of $M$ with respect to the list of pivot column indices $I = (i_1, \dotsc, i_{d'})$ is a $d \times n$ matrix $\text{HNF}(M)$ over $\Z_{m}$ satisfying:
\begin{enumerate}
\item The subgroup of $\Z_{m}^{n}$ generated by the rows of $\text{HNF}_{I}(M)$ is the same as that generated by the rows of $M$;

\item The first $d'$ rows of $\text{HNF}_{I}(M)$ are nonzero, and the remaining rows are zero; 

\item For $k=1,\dotsc, d'$, all entries in (pivot) column $i_{k}$ of $\text{HNF}_{I}(M)$ are zero except for the $k$-th entry, which is the normalized GCD of the entries of $M$ in column $i_{k}$.
\end{enumerate}
Some choices of pivot columns may not be valid, in that the corresponding Hermite normal form may not exist. This is exactly as in the case of row echelon form over a field. For example, there is no Hermite normal form of $\left(\begin{array}{ccc} 1 & 0 & 0 \\ 0 & 0 & 1 \end{array}\right)$ with respect to the pivot columns $1$ and $2$. There is, of course, a Hermite normal form of the preceding matrix with respect to the pivot columns $1$ and $3$, in either order.

\begin{theorem}[{see Buchmann and Neis \cite[Algorithms~3.2 and 3.4, and Theorem~3.5]{buchmannNeis}}] \label{thm:HNF}
Let $M$ be a $d \times n$ matrix over $\Z_{m}$, and let $d'$ be the least number of generators of the subgroup of $\Z_{m}^{n}$ generated by the rows of $M$. Then the Hermite normal form of $M$ with respect to any valid list of $d'$ pivot columns exists and is unique. 

Furthermore, given $M$ and a list $I$ of pivot column indices, there is a polynomial-time algorithm that returns the Hermite normal form of $M$ with respect to $I$ if $I$ is valid, and returns ``invalid pivots'' otherwise.

There is also a polynomial-time algorithm that, given $M$, returns a list of $d'$ pivot columns and the Hermite normal form of $M$ with respect to those pivots.
\end{theorem}

\begin{proof}[Proof of Theorem~\ref{thm:groupcode}]
Let $U, V \leq \Z_{m}^{n}$ be two $\Z_{m}$-codes given by generating sets of size $d$ (which we assume irredundant, without loss of generality). Denote the corresponding $d \times n$ matrices by $A$ and $B$. Use the second algorithm of Theorem~\ref{thm:HNF} to put $A$ into Hermite normal form with respect to some set of pivot columns $I_{A}$ (chosen by the algorithm). We say a $d \times n$ matrix is in ``standard form'' if its left-most $d \times d$ submatrix is diagonal, and each diagonal entry is a canonical generator of some subgroup of $\Z_{m}$. Put $\text{HNF}(A)$ into standard form by permuting its columns so that the pivot columns $I_{A}$ move to the first $d$ columns, and the left-most $d \times d$ submatrix is diagonal. Call the resulting matrix $A'$.

For each choice of subset $I \subseteq [n]$ of size $d$, compute $\text{HNF}_{I}(B)$. If the algorithm of Theorem~\ref{thm:HNF} reveals the indices $I$ to be invalid pivots, the ignore this choice of $I$. Otherwise, permute the columns of $B$ as above to put it into standard form $B'$.

Given a $d \times n$ matrix $M'$ over $\Z_{m}$ in standard form (as $A', B'$), construct the following vertex-and-edge-colored bipartite graph $G_{M'}$: $G_{M'}$ has $d$ vertices in one of its parts and $n-d$ vertices in the other. Among the $d$ vertices, the $i$-th is colored by the $(i,i)$ entry of $M'$. The vertices on the $(n-d)$ side are uncolored. The edge from vertex $i \in [d]$ to vertex $j \in [n-d]$ is colored by $M'_{i, i + j}$. 

We claim that $G_{A'}$ and $G_{B'}$ are isomorphic as bipartite, edge-and-vertex colored graphs if and only if $A$ and $B$ are equivalent. This is essentially the same as in Babai's algorithm (see \cite[Theorem~7.1]{BCGQ}). By combining these isomorphisms with the pre-processing permutations used to compute $A'$ and $B'$, we can easily determine a single group code equivalence and a generating set for the automorphism group of either code $U, V$.

Finally, the coset of bipartite colored graph isomorphisms can be found in $2^{\tilde{O}(\sqrt{n})}$ time \cite{BL83}. Thus the total running time of the algorithm is $O(n^{O(1)}\log^2(m) \binom{n}{d} 2^{\tilde{O}(\sqrt{n})}) \leq (2 + o(1))^{n} \log^2(m)$.
\end{proof}


==> previous.tex <==

The group isomorphism problem \GpI is to determine whether two finite groups, given by their multiplication tables (``Cayley tables''), are isomorphic. For groups of order $n$, the easy $n^{\log n + O(1)}$-time algorithm \cite{FN,Mil78}\footnote{Miller \cite{Mil78} attributes this algorithm to Tarjan.} for the general case of \GpI has barely been improved over the past four decades (it was improved recently to $n^{0.5 \log n + O(1)}$ by Rosenbaum \cite{Rosen2}). The past few years have witnessed a resurgence of activity on this problem \cite{Gal09,CTW10,BCGQ,QST11,Wag11,LW12,BQ,BCQ,Rosen,Rosen2}.
%\footnote{}.
Before introducing these works and our results, we recall why \GpI is an intriguing problem from the complexity-theoretic perspective.

As \GpI reduces to graph isomorphism (\GrI) (see, \eg, the book \cite{struct}), \GpI currently has an intermediate status: it is not $\cc{NP}$-complete unless $\cc{PH}$ collapses \cite{BHZ,babai-moran}, and is not known to be in $\cc{P}$. In addition to its intrinsic interest, resolving the exact complexity of \GpI is a tantalizing question. Further, there is a surprising connection between \GpI and the Geometric Complexity Theory program (see, \eg, \cite{gct_acm} and references therein): techniques from \GpI were used to solve cases of \algprob{Lie algebra isomorphism} that have applications in Geometric Complexity Theory \cite{grochowLie}.

In a survey article \cite{Babaisurvey} in 1995, after enumerating several isomorphism-type problems including \GrI and \GpI, Babai expressed the belief that \GpI might be the only one expected to be in $\cc{P}$.\footnote{The exact quotation from Babai's 1995 survey \cite{Babaisurvey} is: ``None of the problems mentioned in this section, with the possible exception of isomorphism of groups given by a Cayley table, is expected to have polynomial time solution.''} Indeed, in many ways \GpI seems easier than \GrI: there is a simple $n^{\log n+O(1)}$-time algorithm for \GpI, whereas the best known algorithm (see \cite{BL83}) for \GrI takes time $2^{\tilde{O}(\sqrt{n})}$ and is quite complicated. There is a polynomial-time reduction from \GpI to \GrI, yet there is provably no $\cc{AC}^0$ reduction in the opposite direction \cite{CTW10}. Further, \GrI is as hard as its counting version, whereas no such counting-to-decision reduction is known for \GpI. Finally, whereas the smallest standard complexity class known to contain \GrI is $\cc{NP} \cap \cc{coAM}$, Arvind and Tor\'{a}n \cite{AT11} showed that \GpI for solvable groups\footnote{A group is solvable if all its composition factors are abelian.} is in $\cc{NP} \cap \cc{coNP}$ under a plausible assumption, weaker than that needed to show $\GrI \in \cc{coNP}$.

Despite this situation and considerable attention to \GpI, prior to 2009 the actual developments towards polynomial-time algorithms for \GpI essentially stopped at abelian groups. For abelian groups, Kavitha exhibited an $O(n)$-time algorithm \cite{Kav07}, improving Savage's $O(n^{2})$ \cite{Sav80} and Vikas's $O(n \log n)$ \cite{Vik96}. 
The next natural group class after abelian groups---class 2 nilpotent groups\footnote{A group $G$ is nilpotent of class 2 if the quotient $G/Z(G)$ is abelian, where $Z(G)$ is the center of $G$.}---turns out to be formidable.\footnote{Although Garzon and Zalcstein \cite{GZ}, in 1991, solved \GpI for a subclass of nonabelian class 2 nilpotent groups, this subclass seems quite restricted and has not yielded further insights into nilpotent groups since then.}
On the other hand, there is a large body of work in the area referred to as computational group theory (CGT) on practical algorithms for group isomorphism testing.
That line of research typically works on inputs much more succinct than the full Cayley table, while the algorithms are often heuristic.
In the main text, we mostly restrict our attention to works with explicit worst-case analysis. See Appendix~\full{F} for a discussion of the relationship between these two lines of research, as well as works in CGT related to our results.

%Furthermore, several observations indicate that \GpI could be (much) easier than \GrI: (1) the best algorithm for \GrI runs in time $2^{\tilde{O}(\sqrt{n})}$, while $\GpI$ has an easy $n^{\log n+O(1)}$-time algorithm\footnote{Recently, Rosenbaum exhibited an $n^{0.5\log n+o(\log n)}$-time algorithm for solavable groups, building on an idea by Wagner. }, where $n$ is the graph size or the group order. (2) \GrI is self-reducible, namely constructing an isomorphism reduces to deciding the existence of isomorphisms, while \GpI is not know to have this property. Formally, a recent work shows that \GrI cannot be reduced to \GpI via $\AC^0$ reductions.

Beginning in 2009 there were several advances, starting with Le Gall \cite{Gal09}. In \cite{BCQ}, following \cite{BCGQ}, Babai \etal developed a polynomial-time algorithm for groups with no abelian normal subgroups. This suggests the presence of abelian normal subgroups as a bottleneck.\footnote{\label{fn:indecomp} Abelian direct factors, as in $H \times \Z_n$ are not a bottleneck however: Kayal and Nezhmetdinov \cite{KN09} and Wilson \cite{Wil10} gave polynomial-time algorithms to decompose a direct product into its direct factors. For polynomial-time algorithms, one may thus assume that the groups under consideration are \emph{directly indecomposable}: they cannot be written as a direct product of two nontrivial groups.} With this in mind, Babai and Qiao \cite{BQ} developed a polynomial-time algorithm for a special class %\footnote{The group class is referred to as groups with abelian Sylow towers in \cite{BQ}, but we will see that in our context, it corresponds to coprime extensions of abelian groups.}
of non-nilpotent solvable groups, building on \cite{Gal09, QST11}. In \cite{LW12}, Lewis and Wilson took an interesting step towards $p$-group isomorphism: they gave a polynomial-time algorithm for quotients of generalized Heisenberg groups -- a decently large collection of $p$-groups of class 2. In 2013, Rosenbaum \cite{Rosen,Rosen2} exhibited a deterministic $n^{0.25\log n+o(\log n)}$-time algorithm for solvable groups, developing ideas of Wagner \cite{Wag11}. Recently, Rosenbaum developed a general algorithmic technique that brings the time complexity of \GpI to $n^{0.5\log n+O(1)}$ \cite{Rosen2}.


%To summarize, at present it is crucial to understand indecomposable$^{\text{\ref{fn:indecomp}}}$ groups with abelian normal subgroups to develop $n^{o(\log n)}$-time algorithms. 

Given these developments, we are at an interesting crossroads: first, as several nontrivial algorithms have recently been developed, it is reasonable to reflect back to see if there is a common pattern that these algorithms follow. Second, of course we should continue to build on these successes to get more $n^{o(\log n)}$-time algorithms for special group classes. And finally, although class-2 nilpotent groups are widely believed to the bottleneck, this has never been formalized; a reduction from the general case to the nilpotent case would be of great interest.
%the bottleneck case---class 2 nilpotent groups---still remains, and it is desirable to formalize a reduction from the general case to this bottleneck case. 

In this paper we contribute to all three of the above endeavors. Specifically, we propose a general strategy for group isomorphism, which is not only necessary and sufficient for algorithms for \GpI, but also helps to explain in a unified way the polynomial-time algorithms on special group classes \cite{BCGQ, BCQ, Gal09, QST11,LW12,BQ}. We then follow this strategy to develop an $n^{O(\log \log n)}$-time algorithm for a group class proposed in \cite{BCGQ} that is a natural stepping stone towards the general case, and polynomial-time algorithms for several prominent subclasses. In \Sec{cannonHolt} we explain how these results may help to reduce general \GpI to the nilpotent case.

